Scaling up MIMO radar for target detection

This work focuses on target detection in a colocated MIMO radar system. Instead of exploiting the classical temporal domain, we propose to explore the spatial dimension (i.e., number of antennas $M$) to derive asymptotic results for the detector. Specifically, we assume no a priori knowledge of the statistics of the autoregressive data generating process and propose to use a mispecified Wald-type detector, which is shown to have an asymptotic $\chi$-squared distribution as $M\to\infty$. Closed-form expressions for the probabilities of false alarm and detection are derived. Numerical results are used to validate the asymptotic analysis in the finite system regime. It turns out that, for the considered scenario, the asymptotic performance is closely matched already for $M\ge 50$.

==> SectionIV.tex <==
%!TEX root = ICASSP19.tex

\section{The Mismatched Maximum Likelihood (MML) Estimator under dependent data}

The asymptotic behaviour of the MML estimator under the assumption of \textit{i.i.d.} data has been investigated, for the first time, in the seminal works of Huber \cite{Huber} and White \cite{white}. We refer to the recent tutorial paper \cite{SPM} for a detailed discussion about the MML estimator and the Misspecified Cram\'{e}r-Rao Bound (MCRB) under  \textit{i.i.d.} data assumption and for a full list of reference on this topic. However, in radar application, the disturbance experienced by the antenna array is generally characterized by a non-flat PSD, or in other words, the disturbance samples collected from different antennas are generally correlated. Consequently, the results in \cite{Huber,white,SPM} cannot be directly exploited since the i.i.d. assumption is violated.

The extension of the MML theory to the dependent observations has been proposed in \cite{MMLE_dep,white_nl_reg_dep,MMLE_time_series} and, under some weak restriction on the \virg{amount of dependence} allowed among observations, it can be show that the results are consistent with the one obtained for the i.i.d. case. In the following we formalize this concepts by summarizing the main results obtained in \cite{MMLE_dep,white_nl_reg_dep}.

\subsection{General formulation of the misspecified estimation problem under dependent data}
A standard procedure used in point estimation is to recast an estimation problem into a relevant (possibly constrained) optimization problem. If $\mb{x}=\{x_n\}_{n=1}^N$ is the available dataset, characterized by an unknown joint pdf $p_{X_N}$, and $\bar{\bs{\theta}} \in \Theta$ is the parameter vector to be estimated, then an estimate $\hat{\bs{\theta}}$ of $\bar{\bs{\theta}}$ can be obtained as:
\be
\hat{\bs{\theta}} =  \underset{\bs{\theta} \in \Theta}{\mathrm{argmin}} \quad Q_N(\mb{x},\bs{\theta}),\quad \mb{x} \sim p_{X_N}
\ee
where $Q_N(\cdot,\cdot)$ is a suitable objective function. For example, in the i.i.d. case, $Q_N(\cdot,\cdot)$ assumes the form $Q_N(\mb{x},\bs{\theta}) \triangleq \frac{1}{N} \sum\limits_{n=1}^{N} q_n(x_n,\bs{\theta})$. Specifically, the MML estimation under i.i.d. data assumption can be obtained by choosing the log-likelihood function $q_n(x_n,\bs{\theta}) = \ln f_{x_n}(x_n;\bs{\theta})$ as objective function where $f_{x_n}(x_n;\bs{\theta})$ is the assumed, and possibly misspecified, pdf of the observation $x_n$ parametrized by $\bs{\theta} \in \Theta$ \cite{Huber,white}. An alternative approach is to select $q_n(x_n,\bs{\theta})$ on the basis of robustness considerations. Robusteness-driven objective functions $q_n(x_n,\bs{\theta})$ give rise to the celebrated class of $M$-estimators (e.g., \cite{book_Huber,book_Maronna,book_zoubir}). 

When the observations are dependent, a suitable objective function $Q_N(\mb{x},\bs{\theta})$ may be defined as \cite{MMLE_dep}:
\be
\label{obj_fun}
Q_N(\mb{x},\bs{\theta}) \triangleq \ln p_{X_N}(\mb{x}) - \ln f_{X_N}(\mb{x};\bs{\theta}),\quad \mb{x} \sim p_{X_N}
\ee
where, as before, $p_{X_N}(\mb{x})$ indicates the true, but unknown, joint data pdf while $f_{X_N}(\mb{x};\bs{\theta})$ is the assumed, possibly misspecified, joint data pdf. The estimate $\hat{\bs{\theta}}$ obtained by using \eqref{obj_fun} as objective function is:
\be
\label{MMLE_gen}
\hat{\bs{\theta}} = \underset{\bs{\theta} \in \Theta}{\mathrm{argmin}} \left\{{\ln p_{X_N}(\mb{x}) - \ln f_{X_N}(\mb{x};\bs{\theta})}\right\}  = \underset{\bs{\theta} \in \Theta}{\mathrm{argmax}} \ln f_{X_N}(\mb{x};\bs{\theta}), \quad \mb{x} \sim p_{X_N}
\ee
that represents MMLE for dependent data. 

\subsection{The pseudo-true parameter vector}
Let us first define the function $\bar{Q}(\bs{\theta})$ as:
\be
\label{Q_bar}
\bar{Q}_N(\bs{\theta}) \triangleq E_{p_{X_N}}\{Q_N(\mb{x},\bs{\theta})\}.
\ee
In the rest of this work, we assume that the technical assumptions on $\bar{Q}_N(\bs{\theta})$, discussed in \cite[Def. 2.1]{MMLE_dep}, are satisfied. In particular, we will always assume the existence and the uniqueness of the vector $\bs{\theta}_{0,N}$ in the interior of the parameter space $\Theta$, such that:
\be
\bs{\theta}_{0,N} \triangleq \underset{\bs{\theta} \in \Theta}{\mathrm{argmin}} \bar{Q}_N(\bs{\theta}).
\ee

If $Q_N(\mb{x},\bs{\theta})$ defined in \eqref{obj_fun} is used as objective function, then from \eqref{Q_bar}:
\be
\bar{Q}_N(\bs{\theta}) = E_{p_{X_N}}\graffe{\ln \frac{p_{X_N}(\mb{x})}{f_{X_N}(\mb{x};\bs{\theta})}} \triangleq D\tonde{p_{X_N}\parallel f_{X_N|\bs{\theta}}},
\ee
where $D\tonde{p_{X_N}\parallel f_{X_N|\bs{\theta}}}$ represents the Kullback-Leibler (KL) divergence between the true joint data pdf $p_{X_N}$ and the assumed one $f_{X_N|\bs{\theta}}$ as function of the parameter vector $\bs{\theta} \in \Theta$.

Similarly to the i.i.d. case \cite[Assumption 1]{SPM}, let us then define as \textit{pseudo-true parameter vector} the vector $\bs{\theta}_{0,N}$ such that:
\be
\label{pseudo_t}
\bs{\theta}_{0,N} \triangleq \underset{\bs{\theta} \in \Theta}{\mathrm{argmin}} D\tonde{p_{X_N}\parallel f_{X_N|\bs{\theta}}}.
\ee 
It is worth underling that, unlike the i.i.d. case, the pseudo-true parameter in \eqref{pseudo_t} may depend on $N$.

\subsection{Consistency and asymptotic normality of the MMLE under dependent data}
In this Subsection, the asymptotic properties of the MMLE, i.e. its (strong) consistency and asymptotic normality, under dependent data will be provided. The following theorem summarizes the results obtained in \cite{MMLE_dep} (see Theorems 2.2 and 2.4 therein) and generalizes to depended data the statement in \cite[Theo. 2]{SPM} given for the i.i.d. case.

\begin{theorem}{\cite[Theo. 2.2, Theo. 2.3, Theo. 2.4]{MMLE_dep}}
	\label{MMLE_asyn}
	Let $\{x_n: \forall n\}$ be a stationary data generating process such that its ACF satisfy $r_X[m] \triangleq E\{x_{n+m}x^*_n\}=O(|m|^{-\gamma}), m \in \mathbb{Z}, \gamma > 1$ \footnote{Given a real-valued function $f(x)$ and a positive real-valued function $g(x)$, $f(x)=O(g(x))$ if and only if there exists a positive real number $a$ and a real number $x_0$ such that $|f(x)|\leq a g(x),\; \forall x \geq x_0$.}. Let $\mb{x}=\{x_n\}_{n=1}^N$ be a set of $N$ dependent observations extracted from $\{x_n: \forall n\}$ and let $p_{X_N}(\mb{x})$ be their \virg{true} joint pdf. Let $f_{X_N}(\mb{x};\bs{\theta}) \in \mathcal{F}_N$ the assumed joint pdf of the data $\mb{x}$, possibly different form $p_{X_N}(\mb{x})$ for every value of the parameter vector $\bs{\theta} \in \Theta$ and $d=\dim(\bs{\theta})$. Finally, let
	\be
	\label{MMLE_theo}
	\hat{\bs{\theta}} \triangleq \underset{\bs{\theta} \in \Theta}{\mathrm{argmax}} f_{X_N}(\mb{x};\bs{\theta}), \quad \mb{x} \sim p_{X_N},
	\ee
	be the MMLE estimator. Then, the following properties hold:
	\begin{itemize}
		\item Consistency 
		\be
		\hat{\bs{\theta}}\overset{a.s.}{\underset{N\rightarrow \infty}{\rightarrow}}\bs{\theta}_{0,N},
		\ee
		where $\overset{a.s.}{\underset{N\rightarrow \infty}{\rightarrow}}$ indicates the almost sure (a.s.) convergence.
		\item Asymptotic normality
		\be
		\label{asym_norm}
		\sqrt{N}\mb{C}^{-1/2}_{\bs{\theta}_{0,N}}(\hat{\bs{\theta}}-\bs{\theta}_{0,N}) \underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\mb{0},\mb{I}_d},
		\ee
		where $\mb{I}_d$ is the $d \times d$ identity matrix and,
		\be
		\label{C_mat}
		\mb{C}_{\bs{\theta}_{0,N}} \triangleq \mb{A}^{-1}_{\bs{\theta}_{0,N}}\mb{B}_{\bs{\theta}_{0,N}}\mb{A}^{-1}_{\bs{\theta}_{0,N}}
		\ee
		\be
		\label{A_def}
		\quadre{\mb{A}_{\bs{\theta}_{0,N}}}_{i,j} \triangleq N^{-1} E_{p_{X_N}}\graffe{\left. \frac{\partial^2 \ln f_{X_N}(\mb{x};\bs{\theta})}{\partial \theta_i\partial \theta_j}\right|_{\bs{\theta} = \bs{\theta}_{0,N}}} ,
		\ee
		\be
		\label{B_def}
		\quadre{\mb{B}_{\bs{\theta}_{0,N}}}_{i,j} \triangleq N^{-1} E_{p_{X_N}}\graffe{\left. \frac{\partial \ln f_{X_N}(\mb{x};\bs{\theta})}{\partial \theta_i}\right|_{\bs{\theta} = \bs{\theta}_{0,N}} \cdot \left. \frac{\partial \ln f_{X_N}(\mb{x};\bs{\theta})}{\partial \theta_j}\right|_{\bs{\theta} = \bs{\theta}_{0,N}}} ,
		\ee
		for $i,j \in \{i,\ldots,d\}$.
	\end{itemize} 
\end{theorem}
\begin{IEEEproof}
	The proof is given in \cite{white_nl_reg_dep,MMLE_dep}.
\end{IEEEproof}

Firstly, it is important to underline that the requirement about the polynomial decay of the ACF is quite weak, at least for radar applications. This requirement in fact limits the amount of \virg{memory} that a sample $x_n$ of the data generating process has about another sample $x_{n+m}$ at a distance of $m$ lags. Note that the ACF of every finite-order ARMA process decays exponentially fast. So, the previous condition allows processes with a \virg{memory} much longer than ARMA ones \cite{white_nl_reg_dep}. For a more formal and deep discussion about this condition, we refer the reader to \cite{CLT_dep,book_CLT_dep_1,book_CLT_dep_2,bradley2005} and the reference therein. We are now ready to state the following fundamental result. 

It is immediately apparent at the asymptotic behaviour of MMLE $\hat{\bs{\theta}}$ under dependent data given in Theorem \ref{MMLE_asyn} has a strong similarity with its counterpart in the i.i.d. case \cite[Theo. 2]{SPM}. Specifically, it converges (strongly) to the pseudo-true parameter vector $\bs{\theta}_{0,N}$, i.e. the point that minimizes the KL divergence between the true joint data pdf $p_{X_N}(\mb{x})$ and the assumed one $f_{X_N}(\mb{x};\bs{\theta})$. Moreover, the MMLE $\hat{\bs{\theta}}$ is asymptotically normal-distributed with (asymptotic) mean value given by $\bs{\theta}_{0,N}$ and covariance matrix $\mb{C}_{\bs{\theta}_{0,N}}=N^{-1}\mb{A}^{-1}_{\bs{\theta}_{0,N}}\mb{B}_{\bs{\theta}_{0,N}}\mb{A}^{-1}_{\bs{\theta}_{0,N}}$ in \eqref{C_mat}. It is be also noted that the statistical meaning of the matrices $\mb{A}_{\bs{\theta}_{0,N}}$ and $\mb{B}_{\bs{\theta}_{0,N}}$ are exactly the same of the one discussed in \cite{SPM} for the i.i.d. case.

After having discussed the properties of the MMLE, we can move to specify these general framework to the specific misspecification problem at hand presented in subsection \ref{HT_missp}. 


==> SectionVI.tex <==
%!TEX root = ICASSP19.tex

\section{Robust Wald statistic for Scenario $\ref{AR_case}$}

In this Section, we will go back to the main goal of this work: find a decision rule for the HT problem in \eqref{HT_1} whose asymptotic pdf is invariant w.r.t. a misspecification of the pdf of the innovations of the AR(1) data generating process as precisely stated in the Scenario \ref{AR_case}. We show here that such a decision rule exists and it is given by the Misspecified Wald statistic $\Lambda_{MW}(\mb{x})$ that will be defined ahead.

In the following, we show that, under the null hypothesis, $\Lambda_{MW}$ has an asymptotic central $\chi$-square distribution, i.e.
\be
\Lambda_{MW}(\mb{x}|H_0)  \underset{N\rightarrow \infty}{\sim} \chi_2^2(0),
\ee 
so the $P_{FA}$ constraint can be met (at least, asymptotically) even in the presence of the mismatched Scenario \eqref{AR_case}. Moreover, the asymptotic distribution of $\Lambda_{MW}$ under \textit{local alternatives} is also provided and it can be used to approximate the $P_D$ of the misspecified Wald statistic. The tools that we will use to derive this asymptotic results are quite standard (see e.g. \cite[Ch. 9]{Cox} for similar proofs).

Let us start by noticing that the HT problem in \eqref{HT_base_x} can be simply expressed as: 
\be
\label{HT_alpha}
H_0: \; \mb{l}(\bar{\bs{\theta}}) = \tilde{\bs{\alpha}} = \mb{0}_2.
\ee
where, in our case $\mb{l}(\bar{\bs{\theta}})=\quadre{\mb{I}_2,\mb{0}_3}\bar{\bs{\theta}}$ and consequently, its Jacobian matrix in $\bar{\bs{\theta}}$ is simply $\mb{L}_{\bar{\bs{\theta}}} = \quadre{\mb{I}_2,\mb{0}_3}$. Then, the Misspecified Wald statistic related to the null hypothesis in \eqref{HT_alpha} is given by \cite{MMLE_dep,MMLE_time_series}:
\be
\label{Wald_test}
\begin{split}
	\Lambda_{MW}(\mb{x}) &= N\mb{l}^T(\hat{\bs{\theta}})\tonde{\mb{L}_{\hat{\bs{\theta}}}\mb{C}_N(\hat{\bs{\theta}})\mb{L}^T_{\hat{\bs{\theta}}}}^{-1}\mb{l}^T(\hat{\bs{\theta}})\\
	& =  N \hat{\tilde{\bs{\alpha}}}^T\tonde{\quadre{\mb{C}_N(\hat{\bs{\theta}})}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}}^{-1}\hat{\tilde{\bs{\alpha}}},
\end{split}
\ee
where, as the notation suggests, $\quadre{\mb{C}_N(\hat{\bs{\theta}})}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}$ is the top-left, $2 \times 2$ submatrix of $\mb{C}_N(\hat{\bs{\theta}})$ in \eqref{C_N}, while $\hat{\bs{\theta}}=[\hat{\bs{\theta}}]_{1:2}$ is the MMLE estimator \eqref{MMLE_gauss} of $\tilde{\bar{\bs{\alpha}}}$.

\subsection{Asymptotic distribution of $\Lambda_{MW}$ under $H_0$}
It can be shown that under the null hypothesis $H_0$, $\Lambda_{MW}$ has an asymptotic central $\chi$-square distribution.

Let us define the vector
\be
\bar{\bs{\theta}}_{H_0} \triangleq (\mb{0}_2,\tilde{\bar{\bs{\rho}}},\bar{\sigma}^2)^T,
\ee
as the true parameter vector under the null hypothesis. 

Under $H_0$, from Theorem \ref{Theo_MML_dep}, we have that:
\be
\hat{\bs{\theta}}\overset{a.s.}{\underset{N\rightarrow \infty}{\rightarrow}}\bar{\bs{\theta}}_{H_0},
\ee
\be
\label{norm_alpha}
\sqrt{N}\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}} \underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\mb{0},\mb{I}_2}.
\ee

For Hermitian and positive-definite matrices, the inverse operator and the principal square root are both continuous operators (see e.g. \cite{square_root_cont}), then their composition is continuous. Then, from \eqref{conv_C_est} and by using the Continuous Mapping Theorem \cite[Theo. 2.7]{Billi}, we have that:
\be
\label{conv_C_est_root}
\mb{C}_N^{-1/2}(\hat{\bs{\theta}}) - \mb{C}^{-1/2}_{\bar{\bs{\theta}}_{H_0}} \overset{a.s.}{\underset{N\rightarrow \infty}{\rightarrow}} \mb{0}.
\ee

Let us rewrite the test in \eqref{Wald_test} as:
\be
\Lambda_{MW}(\mb{x}|H_0) = \tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}^T\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}.
\ee

Finally, from \eqref{norm_alpha} and \eqref{conv_C_est_root}, by a direct applications of the Slutsky's Lemma, we immediately obtain that:
\be
\label{asy_H0_MWT}
\Lambda_{MW}(\mb{x}|H_0) = {\underbrace{\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}}_{\underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\mb{0},\mb{I}_2}}}^T\underbrace{\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}}_{\underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\mb{0},\mb{I}_2}} \underset{N\rightarrow \infty}{\sim} \chi_2^2(0),
\ee  
where $\chi_2^2(0)$ indicates a central $\chi$-squared random variable with two degrees of freedom.

\subsection{Asymptotic distribution of $\Lambda_{MW}$ under local alternatives}

Suppose that the alternatives to $H_0$ is of the from:
\be
\label{alter}
H_1: \; \tilde{\bs{\alpha}} = \frac{\mb{d}}{\sqrt{N}}, \quad \mb{d} \in \mathbb{R}^2.
\ee 

Let us define the vector
\be
\bar{\bs{\theta}}_{H_1}^{(N)} \triangleq (\mb{d}/\sqrt{N},\tilde{\bar{\bs{\rho}}},\bar{\sigma}^2)^T,
\ee
as the true parameter vector under local alternatives. Note that
\be
\label{lim_theta}
\lim_{N\rightarrow\infty}\bar{\bs{\theta}}_{H_1}^{(N)} = \bar{\bs{\theta}}_{H_0}.
\ee

If the matrices $\mb{A}_{\bs{\theta}}$ and $\mb{B}_{\bs{\theta}}$, defined in \eqref{A_def} and \eqref{B_def} respectively, are continuous in a neighbourhood of $\bar{\bs{\theta}}_{H_0}$, then $\mb{C}_{\bs{\theta}}$ is continuous in a neighbourhood of $\bar{\bs{\theta}}_{H_0}$ as well. Then, from \eqref{lim_theta}:
\be
\label{lim_C}
\lim_{N\rightarrow\infty}\mb{C}_{\bar{\bs{\theta}}_{H_1}^{(N)}} = \mb{C}_{\bar{\bs{\theta}}_{H_0}}.
\ee

Under $H_1$ in \eqref{alter}, from Theorem \ref{Theo_MML_dep}, we have that:
\be
\hat{\bs{\theta}}\overset{a.s.}{\underset{N\rightarrow \infty}{\rightarrow}}\bar{\bs{\theta}}^{(N)}_{H_1},
\ee
\be
\label{norm_alpha_H1}
\sqrt{N}\quadre{\mb{C}_{\bar{\bs{\theta}}^{(N)}_{H_1}}}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\tonde{\hat{\tilde{\bs{\alpha}}} - \mb{d}/\sqrt{N}} \underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\mb{0},\mb{I}_2}
\ee

As before, by using the Continuous Mapping Theorem \cite[Theo. 2.7]{Billi} and the limiting results in \eqref{lim_C}, we have that:
\be
\label{conv_C_est_root_H1}
\mb{C}_N^{-1/2}(\hat{\bs{\theta}}) - \mb{C}^{-1/2}_{\bar{\bs{\theta}}^{(N)}_{H_1}} \underset{N\rightarrow \infty}{=} \mb{C}_N^{-1/2}(\hat{\bs{\theta}}) - \mb{C}^{-1/2}_{\bar{\bs{\theta}}_{H_0}} \overset{p_{X_N}}{\underset{N\rightarrow \infty}{\rightarrow}} \mb{0}.
\ee

Let us rewrite the test in \eqref{Wald_test} as:
\be
\Lambda_{MW}(\mb{x}|H_1) = \tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}^T\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}.
\ee

Finally, from \eqref{norm_alpha_H1} and \eqref{conv_C_est_root_H1}, by a direct applications of the Slutsky's Theorem, we immediately obtain that:
\be
\label{asy_H1_MWT}
\Lambda_{MW}(\mb{x}|H_1) = {\underbrace{\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}}_{\underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\mb{d},\mb{I}_2}}}^T\underbrace{\tonde{\sqrt{N}\quadre{\mb{C}_N(\hat{\bs{\theta}})}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\hat{\tilde{\bs{\alpha}}}}}_{\underset{N\rightarrow \infty}{\sim} \mathcal{N}\tonde{\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1/2}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\mb{d},\mb{I}_2}} \underset{N\rightarrow \infty}{\sim} \chi_2^2\tonde{\mb{d}^T\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\mb{d}}.
\ee 

This result the can be used to approximate the power of the test, i.e. the $P_D$. To do this, it is enough to put $\mb{d} \equiv \sqrt{N}\tilde{\bar{\bs{\alpha}}}$. Then, we have:
\be
\Lambda_{MW}(\mb{x}|H_1) \underset{N\rightarrow \infty}{\sim} \chi_2^2\tonde{N\tilde{\bar{\bs{\alpha}}}^T\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\tilde{\bar{\bs{\alpha}}}}.
\ee
Finally, using the properties of the non-central $\chi$-squared distribution with $2$ dof \cite{non_cenrtal_CDF}, a closed form expression of the asymptotic probability of detection in \eqref{PD_def}, can be expressed as:
\be
P_D(\lambda) = Q_1\tonde{\sqrt{N\tilde{\bar{\bs{\alpha}}}^T\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\tilde{\bar{\bs{\alpha}}}},\sqrt{\lambda}},
\ee
where $Q_1(\cdot,\cdot)$ is the Marcum $Q$ function of order 1. Finally, by combining the two results in \eqref{asy_H0_MWT} and \eqref{asy_H1_MWT} and the relation in \eqref{asy_dist_H0}, we can express the probability of detection as function of the nominal probability of false alarm:
\be
\label{closed_form_ROC}
P_D(\overline{P_{FA}}) = Q_1\tonde{\sqrt{N\tilde{\bar{\bs{\alpha}}}^T\quadre{\mb{C}_{\bar{\bs{\theta}}_{H_0}}}^{-1}_{\tilde{\bs{\alpha}},\tilde{\bs{\alpha}}}\tilde{\bar{\bs{\alpha}}}},\sqrt{-2\ln \overline{P_{FA}}}}.
\ee 
Note that, as proved in \cite{Q_fun}, the Marcum $Q_1$-function is strictly increasing with the first argument and strictly decreasing with the second argument.



==> SectionVII.tex <==
%!TEX root = ICASSP19.tex

\section{Simulation results}

Simulation parameters:
\begin{itemize}
	\item $\bar{\rho} = |\rho|e^{j2\pi\nu_c}$, where $\nu_c = 0.25$ and $|\rho|=0.9$, $|\rho|=0.7$, $|\rho|=0.3$,
	\item For $n=1,\ldots,N$, we set $v_n = e^{j2\pi\nu(n-1)}$ where $\nu=0.23$,
	\item $\overline{P_{FA}} = 10^{-4}$,
	\item Number of independent Monte Carlo trials: $10^6$.
\end{itemize}

\begin{figure}[H]
	\centering
	\includegraphics[height=7cm]{images/PFA_vs_sqrtN_07_03_09.eps}
	\caption{Estimated and nominal $P_{FA}$. The threshold has been set according to a nominal $P_{FA}$ of $10^{-4}$.}
	\label{fig:Fig1}
\end{figure}

\begin{figure}[H]
	\centering
	\includegraphics[height=7cm]{images/PD_vs_sqrtN_07_03_09.eps}
	\caption{Estimated and nominal $P_{D}$. The threshold has been set according to a nominal $P_{FA}$ of $10^{-4}$. The Signal-to-Noise Ratio is $SNR=-10 dB$ }
	\label{fig:Fig2}
\end{figure}

\begin{figure}[H]
	\centering
	\includegraphics[height=7cm]{images/PFA_vs_lambda_rho_07.eps}
	\caption{Estimated and nominal $P_{FA}$. The absolute value of the one-lag coefficient is $|\rho|=0.7$. The threshold has been set according to a nominal $P_{FA}$ of $10^{-4}$. The number of samples is $N=1000$ }
	\label{fig:Fig3}
\end{figure}

\begin{figure}[H]
	\centering
	\includegraphics[height=7cm]{images/PD_vs_lambda_rho_07.eps}
	\caption{Estimated and nominal $P_{D}$. The absolute value of the one-lag coefficient is $|\rho|=0.7$. The number of samples is $N=1000$. The threshold has been set according to a nominal $P_{FA}$ of $10^{-4}$. The Signal-to-Noise Ratio is $SNR=-10 dB$ }
	\label{fig:Fig4}
\end{figure}
